Hybrid Task Cascade for Instance Segmentation

Cascade is a classic yet powerful architecture that has boosted performance on various tasks. However, how to introduce cascade to instance segmentation remains an open question. A simple combination of Cascade R-CNN and Mask R-CNN only brings limited gain. In exploring a more effective approach, we find that the key to a successful instance segmentation cascade is to fully leverage the reciprocal relationship between detection and segmentation. In this work, we propose a new framework, Hybrid Task Cascade (HTC), which differs in two important aspects: (1) instead of performing cascaded refinement on these two tasks separately, it interweaves them for a joint multi-stage processing; (2) it adopts a fully convolutional branch to provide spatial context, which can help distinguishing hard foreground from cluttered background. Overall, this framework can learn more discriminative features progressively while integrating complementary features together in each stage. Without bells and whistles, a single HTC obtains 38.4 and 1.5 improvement over a strong Cascade Mask R-CNN baseline on MSCOCO dataset. Moreover, our overall system achieves 48.6 mask AP on the test-challenge split, ranking 1st in the COCO 2018 Challenge Object Detection Task. Code is available at: https://github.com/open-mmlab/mmdetection.

==> sections/introduction_bak.tex <==
% !TEX root = ../main.tex

\section{Introduction}
% Instance segmentation is a fundamental task in computer vision. Compared with
% object detection, it is more challenging since it requires instance-level
% mask prediction other than merely bounding box prediction.
% With instance masks, computers can have a more subtle perception of images and videos,
% which benefits lots of real-world applications like autonomous driving and video surveillance.

Instance segmentation is a fundamental computer vision task that requires the per-pixel labeling of objects at instance level, which gives rise to a more detailed and comprehensive visual understanding.
An accurate and robust instance segmentation system benefits lots of real-world applications including autonomous driving and video surveillance. 
However, there are several major challenges towards achieving this goal.
Firstly, instance segmentation involves the pixel-wise localization of object instances that usually undergo deformation, occlusion and scale changes. Therefore, a powerful representation that adaptively handles these scenarios is highly desirable.
Secondly, object instances also co-exist within the cluttered scenes.
The spatial contexts that discriminate object foreground and cluttered background thus become necessary.  
To substantially push the performance in this area, a powerful architecture that learns robust and discriminative features is at desire.

% Cascaded or multi-stage architectures have been adopted by object detection methods for a long time,
% and the recently proposed Cascade R-CNN~\cite{cai18cascadercnn} brings it to a new level in the era of CNN-based approaches.
% There are two fatal factors in the design of Cascade R-CNN, progressive refinement and adaptive distribution.
% Thanks to the connections between consecutive stages, the output of a stage is fed to the next one for higher quality refinement.
% To better match the progressively improved hypotheses, each stage is trained with sampled proposals of increasing IoU thresholds.
% %
% Though the aforementioned cascaded structure presents its strength on improving detection qualities,
% it is originally designed for object detection and how to apply it to instance
% segmentaion remains an open problem.
% There are an early attempt\cite{dai2016instance} that also involves multiple stages,
% but it mainly focuses on arranging multiple tasks in an end-to-end pipeline.

Cascade is a classic yet powerful architecture that has boosted performance on various tasks by multi-stage refinement.
Recently, Cascade R-CNN~\cite{cai18cascadercnn} bring this idea into object detection and achieved promising results.
Two key ingredients explain the success of Cascade R-CNN: (1) progressive refinement of predictions; (2) adaptive handling of training distributions.
On the one hand, the output of each stage is fed into the next stage for higher quality refinement.
On the other hand, the training data of each stage is sampled with increasing IoU thresholds, which inherently handles different training distributions.
Though being effective on detection tasks, integrating the idea of cascade into instance segmentation is not trivial.
A direct combination of Cascade R-CNN and Mask R-CNN~\cite{he2017mask} only brings limited gain.

% Motivated by the success of cascaded architectures, we propose Hybrid Task Cascade, a new instance segmentation framework.
To bridge this gap, we investigate effective cascade for instance segmentation in this work by proposing a novel architecture, Hybrid Task Cascade (HTC).
It incorporates multi-task and stage-wise architectures in a single pipeline,
where branches for different tasks and stages for increasing quality levels are organized in a hybrid way.
% component 1
Primarily, we add a mask branch in each stage following Mask R-CNN~\cite{he2017mask},
which is a straight forward adaption of Cascade R-CNN to the instance segmentation task.
%
% component 2
Furthermore, we investigate the information flow through different stages.
In Cascade R-CNN, the output bounding boxes of a stage are used to crop features
and compute regression targets for the next stage.
The currently stage is aware of the information of the last stage in two aspects: 
1) the learning target is closely related to the output of last stage;
2) the input feature is jointly determined by the output last stage and backbone.
Following such conventions, we introduce direct connections between mask branches in adjacent stages.
In each stage, given a set of bounding boxes, features are not simply extracted
from the backbone feature maps, but also from the mask branch of the last stage.
These connections benefits progressive refinement by creating an information flow through mask branches of different stages.

% component 3
Spatial contexts also serve as a strong complement to instance segmentation cascade.
Specifically, we introduce complementary information by adding a semantic segmentation branch.
This branch adopts the fully convolutional structure and is supervised by pixel-level stuff annotations.
As a complement to box and mask branches, it encodes more contextual information and 
is more discriminative on background regions.
However, a na\"{\i}ve multi-task learning is observed to only bring few gains to the mask prediction.
Instead, here we combine the semantic and box branches in each stage by fusing their internal features.

Hybrid Task Cascade (HTC) is easy to implement and can be trained end-to-end.
Without bells and whistles, it achieves XX\% higher mask AP with a ResNet-50 backbone than Mask R-CNN baseline on the challenging MS COCO dataset.
Together with better backbones and other common components,~\eg, deformable convolution,
multi-scale training and testing, model ensembling, we achieve 49.0 mask AP on test-dev dataset,
which is 2.3\% higher than the winning approach~\cite{liu2018path} of COCO Challenge 2017.

% The main contributions of this work lie in several aspects:
% (1) the Hybrid Task Cascade, which provides a solution to applying cascaded architectures in the task of instance segmentaion,
% (2) the introduction of connections through multi-stage mask branches, revealing the importance of direct information flow to progressive refinement,
% (3) the combination of complementary semantic features.

Our main contributions are summarized as follows:
(1) We propose Hybrid Task Cascade (HTC), which effectively integrates cascade into instance segmentation by interweaving detection and segmentation features together for a joint multi-stage processing.
(2) We demonstrate that spatial contexts benefit instance segmentation by discriminating foreground objects from background clutters.
(3) Our overall system achieves the best performance in MS COCO 2018 instance segmentation Challenge.
(4) We contribute a highly-optimized detection/segmentation codebase to this community, which modularly implements and comprehensively benchmarks various state-of-the-art detection/segmentation networks to facilitate future research.

